On the Robustness of LDP Protocols for Numerical Attributes under Data Poisoning Attacks

Recent studies reveal that local differential privacy (LDP) protocols are vulnerable to data poisoning attacks where an attacker can manipulate the final estimate on the server by leveraging the characteristics of LDP and sending carefully crafted data from a small fraction of controlled local clients. This vulnerability raises concerns regarding the robustness and reliability of LDP in hostile environments. In this paper, we conduct a systematic investigation of the robustness of state-of-the-art LDP protocols for numerical attributes, i.e., categorical frequency oracles (CFOs) with binning and consistency, and distribution reconstruction. We evaluate protocol robustness through an attack-driven approach and propose new metrics for cross-protocol attack gain measurement. The results indicate that Square Wave and CFO-based protocols in the Server setting are more robust against the attack compared to the CFO-based protocols in the User setting. Our evaluation also unfolds new relationships between LDP security and its inherent design choices. We found that the hash domain size in local-hashing-based LDP has a profound impact on protocol robustness beyond the well-known effect on utility. Further, we propose a zero-shot attack detection by leveraging the rich reconstructed distribution information. The experiment show that our detection significantly improves the existing methods and effectively identifies data manipulation in challenging scenarios.

==> 1_introduction.tex <==
\section{Introduction}

Local Differential Privacy is the \textit{de facto} standard for data privacy in distribution environment. There are many LDP protocols for various statistical tasks such as frequency estimation \cite{wang2020locally, wang2017locally, wang2018locally}, distribution estimation \cite{li2020estimating, murakami2019utility}, key-value data collection \cite{gu2020pckv, ye2019privkv, ye2021privkvm} and graph statistic estimation \cite{imola2021locally, ye2020lf}. LDP has also been deployed in companies like Google \cite{erlingsson2014rappor}, Apple \cite{apple} and Microsoft \cite{ding2017collecting}.

Recent studies show that LDP protocols are vulnerable to poisoning attacks.  In LDP context, users report data to the server.  All LDP protocols require the usage of some perturbation algorithm $\Psi(x): \mathcal{D} \rightarrow \hat{\mathcal{D}}$, where $\mathcal{D}$ is the domain of user's values, and $\hat{\mathcal{D}}$ is the output domain of $\Psi$.  A user with private value $x$ would report $\Psi(x)$.  
Some of these users may be malicious or compromised by an attacker and intentionally report wrong results.  If a malicious user with private value $x$ reports $\Psi(x')$, then this behavior is indistinguishable from a user whose true value is $x'$.  This is considered the baseline of poisoning attacks.  However, malicious users can directly choose values in $\hat{\mathcal{D}}$ that best achieve the attack objective and report these carefully chosen values.  Different LDP protocols may have very different degrees of vulnerability to such attacks.  

%Recent studies show there are security issues in LDP protocols. The estimated results of LDP can be manipulated under data poisoning attack. In LDP context, there are two types of data poisoning attack: 1) input poisoning attack and 2) output poisoning attack. Input poisoning attack is straightforward and the attacker directly injects fake data into the input domain of LDP protocol to skew the estimates, which is also considered as the baseline. Output poisoning attacker can craft fake values using characteristic of LDP protocols and obtain better attack performance. Due to the advanced attack efficacy, most existing works focus on output poisoning attack. In particular, Cheu \textit{et al.} \cite{cheu2021manipulation} studied \textit{untargeted attack} that allows an attacker to compromise a group of legitimate users and inject false data to degrade the overall performance of LDP protocols. Wu \textit{et al.} \cite{wu2021poisoning} and Cao \textit{et al.} \cite{cao2021data} studied the optimal \textit{targeted attack} to maximally promote the associated statistics on attacker-chosen items or key-value data.

In this paper, we study the effect of poison attacks against LDP protocols for numerical data.  In the literature, Cheu \textit{et al.} \cite{cheu2021manipulation} studied \textit{untargeted attack} against frequency oracles in categorical data. Wu \textit{et al.} \cite{wu2021poisoning} and Cao \textit{et al.} \cite{cao2021data} studied \textit{targeted attacks} to maximally promote the associated statistics on attacker-chosen items or key-value data. \li{Different from maximizing the statistics, Li \textit{et al.} \cite{li2022fine} investigated the \textit{fine-grained attack} to simultaneously manipulate the mean and variance to target values.} \sun{include our fine-grained attacks? and discuss it related work as well} \li{To the best of our knowledge, we are the first to study poisoning attacks against LDP protocols for numerical data.} \sun{mean/variance are also numerical? and key value?} We aim to answer the following research questions:  (1) What are the most effective attacks against different LDP protocols? \sun{I think it is too broad}  (2) How different LDP protocols compare in terms of robustness against poisoning attacks?  Typically LDP protocols are compared based on estimation accuracy; robustness adds another interesting dimension one should consider when choosing a LDP protocol. \sun{what is the definition of robustness?}  (3) How to detect such poisoning attacks?

\li{natural robustness and active detection.}

For attack objective, we focus on increasing (or decreasing) estimated mean.  Mean estimation is the task that several protocols are specifically designed for, and can be used to estimate other statistical quantities, such as the variance.  
To evaluate the effectiveness of a mean-manipulation attack, a natural metric is to measure the mean gain $| \hat{\mu}_a - \mu |$, where $\hat{\mu}_a$ is the estimated mean after attack. However, mean gain is influenced by factors such as the privacy parameter $\epsilon$ and the fraction of users that are assumed to be malicious; it does not directly yield the strength of an attack or the robustness of a LDP protocol.  We propose a new metric called mean gain ratio (MGR). The key intuition is to measure the ratio of the mean gain from the proposed attack, i.e., $| \hat{\mu}_a - \mu |$, to the mean gain of the baseline, i.e., $| \hat{\mu}_a^{base} - \mu |$. Due to the LDP noise, the mean gain of the baseline attack is random and attacks with the same $\hat{\mu}_a$ may have different measurement. Therefore, we substitute the term $\hat{\mu}_a^{base}$ with the skewed mean in the input domain since the estimated mean in a well-designed LDP protocol is unbiased and close to the mean in the input domain. By this substitution, the denominator of MGR is a constant.  An MGR value of $1$ means that the attack is no more effective than the baseline and should not be a concern.  On the other hand, a high MGR value, such as $10$ or higher, is highly concerning.  Thus, we can easily use MGR to compare different attacks as well as different LDP protocols. 

We study four state-of-the-art LDP mechanisms for numerical data.  SR \cite{duchi2018minimax} and PM \cite{wang2019collecting} were designed for mean estimation.  CFOB \cite{li2020estimating} and SW \cite{li2020estimating} were designed to output a distribution, from which one can compute the mean.   In~\cite{li2020estimating}, it was demonstrated that SW can give more accurate estimates for mean and variance. 


We formulate the attack as an optimization problem.  
Moreover, we theoretically and empirically study the effectiveness of the attack. Theoretically, we find it is challenging to solve the optimal fake values for SW mechanism since the output of SW mechanism depends on distribution of the underlying true data and the attack efficacy is unpredictable to the attacker. 
% Prior work demonstrated the security-privacy tradeoff in LDP protocols for categorical and numerical data \sun{it is not accurate for key value and does not hold for fine grained.}. Specifically, smaller $\epsilon$ provides higher privacy but weaker security of LDP. However, we find such tradeoff does not hold for SW mechanism, which further complicates the attack since even under small $\epsilon$, the security of SW may be not weak.
\li{Prior work studied the relationship between the security of LDP protocols and privacy budget $\epsilon$ varies under different attacks. Specifically, under targeted attacks, recent works \cite{cheu2021manipulation, cao2021data} show the security-privacy tradeoff for LDP protocols: smaller $\epsilon$ provides higher privacy but weaker security. Under fine-grained attack \cite{li2022fine}, smaller $\epsilon$ provides stronger security because it leads to larger noise and greater error between estimated results and target values. This property is called security-privacy consistency. However, we find neither tradeoff nor consistency holds for SW mechanism, which further complicates the attack since it is challenging to determine when the security of SW is weak.}
Empirically, we evaluate the attack on multiple datasets. Due to the lack of optimal attack, we intuitively inject four types of large values (or small values) to SW for increasing the mean (or decreasing the mean). The results show the best attack type varies under different datasets and $\epsilon$ and there is no optimal attack. Besides, the MGR of attack on SW is lower than other mechanisms in most cases, indicating SW can naturally resist the attack.


%for mean estimation under the poisoning attack. We first investigate the optimal attack on mean estimation. In our attack, the attacker can compromise a part of genuine users and use them to send carefully-crafted fake values to the server, with the goal to maximally increase or decrease the estimated mean. We formulate the attack as an optimization problem whose objective function is to maximize the attack efficacy and whose solution are the fake values. To evaluate the attack, a natural metric is to measure the mean gain $| \hat{\mu}_a - \mu |$, where $\hat{\mu}_a$ is the estimated mean after attack. However, mean gain can only indicate how much the attack increase/decrease the mean, but cannot evaluate how much the attack outperforms the baseline. To address this problem, we propose a new metric called mean gain ratio (MGR). The key intuition is to measure the ratio of the mean gain from the proposed attack, i.e., $| \hat{\mu}_a - \mu |$, to the mean gain of the baseline, i.e., $| \hat{\mu}_a^{base} - \mu |$. Due to the LDP noise, the mean gain of the baseline attack is random and attacks with the same $\hat{\mu}_a$ may have different measurement. Therefore, we substitute the term $\hat{\mu}_a^{base}$ with the skewed mean in the input domain since the estimated mean in a well-designed LDP protocol is unbiased and close to the mean in the input domain. By this substitution, the denominator of MGR is a constant. Thus, MGR can not only measure which attack performs better, but can also measure how much the attack outperforms the baseline.

Attack detection strategy is widely used to mitigate poisoning attacks. Generally, the defender uses information about genuine users or true data as the benchmark and determines if the attack occurs \cite{gong2014sybilbelief, jia2017random}. However, in LDP scenario, there is no benchmark. Trapped in this challenge, existing mitigations are not practical since they either rely on strong assumptions about the true data or only work well in worst cases \cite{cao2021data, wu2021poisoning}. To further enhance the LDP security, we also investigate the attack detection framework for LDP protocols for mean estimation. The key intuition is to leverage the distribution information returned by LDP protocols to construct the benchmark for detection. Specifically, we first estimate the data distribution from the noisy report and synthesize data follow this distribution. Given the synthetic data, we reconstruct two groups of noisy results by LDP perturbation and calculate a group of distances between them as benchmark since they are not polluted. Then we calculate a group of distances between the reported result and reconstructed results and statistically analyze the similarity between it with the benchmark distance group by KS test, which is a hypothesis test method to determine if the distributions of two groups of samples are similar. \sun{might need to be concise.} When these two distance groups are similar, the reported result is not polluted. We note that not all LDP mechanisms can return the distribution information and our framework cannot enhance security for such mechanisms. \sun{no need to mention here} For example, SR and PM only return a single value as estimate of mean. We evaluate the detection framework on multiple datasets and the results show the our detection can effectively capture the attack.


% Attack detection is a widely-used mitigation for data poisoning attack. Generally, the defender uses information about genuine users or true data as the benchmark and determine if the attack occurs \cite{gong2014sybilbelief, jia2017random}. Unfortunately, these methods cannot be directly applied in LDP scenarios because the data collector cannot access the information about true data. 
% To address this challenge, Wu \textit{et al.} \cite{wu2021poisoning} assume a part of genuine users' data is known and train a one-class classifier by these data to detect attack to LDP protocols for key-value collection. In order to detect attack for frequency estimation, Cao \textit{et al.} \cite{cao2021data} find the upper bound of the frequency anomaly threshold by traversing all possible true frequencies, and attack occurs when the noisy frequency of item is larger than the bound. 
% Trapped in this challenge, previous countermeasures for LDP protocols are not practical because they either rely on strong assumption about the true data or only work well in worst cases \cite{cao2021data, wu2021poisoning}. To address this challenge, 

We summarize the contribution below.
\begin{enumerate}
    \item We perform the first systematic study on optimal poisoning attack to LDP protocols for mean estimation, and analyze the robustness of a family of LDP mechanisms under the attack.
    
    \item We propose a new metric for attack efficacy. This metric considers the baseline attack \sun{remind what is baseline} and can show how much the attack outperforms the baseline.
    
    \item We design a new detection framework for poisoning attack. It can effectively detect the attack without knowing the ground truth.
    
    \item We comprehensively evaluate the attack and the detection on three real-world datasets and one synthetic dataset. The empirical study shows SW mechanism can naturally resist the proposed attack, and the framework can effectively capture the attack.
\end{enumerate}

==> 1_introduction_v2.tex <==
\section{Introduction}
Local differential privacy (LDP) is the \textit{de facto} standard for privacy-protective data collection in a distribution environment for various statistical tasks such as frequency estimation \cite{wang2020locally, wang2017locally, wang2018locally, erlingsson2014rappor, acharya2019hadamard, bassily2015local}, distribution estimation \cite{li2020estimating, murakami2019utility, duchi2018minimax}, key-value data collection \cite{gu2020pckv, ye2019privkv, ye2021privkvm} and graph statistic estimation \cite{imola2021locally, ye2020lf}. It has been deployed in many commercial products by Google \cite{erlingsson2014rappor}, Apple \cite{apple} and Microsoft \cite{ding2017collecting}. 

Recent studies have shown that LDP protocols are vulnerable to data poisoning/manipulation attacks~\cite{cheu2021manipulation, cao2021data, wu2021poisoning, li2022fine}, where adversary-controlled clients can report fake values to skew the estimates on the server.
One important setting in LDP is when the data to be collected are ordinal or numerical by nature, e.g., income, age, the amount of time spent viewing a certain page, etc. A numerical domain consists of values that have a meaningful total order. Therefore, the main objective for numerical data is to estimate the distribution, since it is a primary statistic from which other statistical properties can be computed without additional privacy costs. However, prior work \cite{li2022fine, cheu2021manipulation} focused on poisoning attacks on some statistical sub-tasks, such as mean and variance estimation. The attack effect on the distribution estimation and the robustness of the corresponding LDP protocols have not been fully understood. To bridge the gap, we intend to advance the knowledge regarding the robustness of LDP in the numerical domain in the presence of data distribution manipulation attacks. We aim to answer the following research questions:

% \begin{itemize}
%     \item 

\mysubpara{RQ1.} For each state-of-the-art numerical LDP protocol under investigation, how to effectively conduct poisoning attacks against it?  
    
    % \item
\mysubpara{RQ2.} How do different LDP protocols compare in terms of robustness against poisoning attacks?  A protocol is less robust than another if, under the same setting, the adversary can induce more impact on the estimated statistical quantity.  While LDP protocols are often compared based on versatility (what kinds of statistics can be estimated from the protocol) and estimation accuracy, robustness adds another interesting and important dimension that one should consider when choosing an LDP protocol.  
    
    % \item
\mysubpara{RQ3.} How to detect such poisoning attacks?  Since in different LDP protocols clients report different kinds of information, for some protocols it would be easier to detect poisoning attacks. Ideally, we desire a protocol that is accurate, versatile, robust, and for which one can deploy effective detection. 
% \end{itemize}


Two types of LDP protocols exist for distribution estimation, each based on different techniques. The first one is based on categorical frequency oracle with binning and consistency. These protocols first bin the numerical attributes and then apply CFOs for binned attributes to estimate the histogram of the data. Due to the noise in LDP, the histogram could not be a valid distribution (e.g., there exist negative values in the histogram). Thus, the protocols further apply post-processing methods to make the estimate consistent with the definition of distribution. We study three state-of-the-art CFOs including \textbf{HST} \cite{cheu2021manipulation}, \textbf{OUE} and \textbf{OLH} \cite{wang2017locally}. HST and OLH depend on public hash functions selected by the server or the user, leading to the \textit{Server} setting and \textit{User} setting respectively.
The other is to directly recover the distribution. We study \textbf{SW}~\cite{li2020estimating}, a representative mechanism in this category.
In SW, the server considers the ordinal nature of the numerical domain and uses Expectation Maximization with Smoothing to reconstruct the distribution given noisy reported values.

To study the robustness of each protocol under data manipulation, we focus on \textbf{Distribution-Shift Attacks} in which the adversary aims to shift the estimated distribution to the right-most end. Intuitively, we may have similar observations for shifting the distribution to the left side.
To evaluate the effectiveness of the attack, we derive the metric \textbf{Absolute Shift Gain} (\ASG) inspired by Wasserstein distance to quantify the extent to which the distribution is shifted towards the right side. Larger \ASG indicates the distribution is shifted closer to the right end. To further minimize the influence of related attack factors, such as the number of malicious users and the ground truth distribution, we also refer to a second metric \textbf{Shift Gain Ratio} (\SGR), which is defined to be the ratio of \ASG of the proposed attack to the \ASG of a baseline attack. In the baseline attack, malicious users follow the LDP protocol but send the maximum allowed input value $x_{\max}$ to maximally skew the distribution. The baseline attack is indistinguishable from the case where  the true input of a group of users are also $x_{\max}$. Therefore, the impact of the baseline is the same on any LDP mechanism that produces an unbiased estimation. $\SGR > 1$ indicates the attack outperforms the baseline, and the larger the metric, the better the attack performance.

Our investigation approaches the LDP security from a new perspective to reveal more implications of LDP mechanism design on protocol robustness instead of only the impact of privacy budget $\epsilon$ on the LDP security. For instance, Our theoretical analysis shows a tradeoff between security and hash domain size of HST and OLH. When a larger hash domain size is set, the protocols are more vulnerable to the attack. We compare the robustness among the studied LDP protocols. While maximizing the reported value's contribution to the frequency of the largest value in the domain can effectively shift the distribution with the mechanisms based on binning and consistency, we find that applying the same attack strategy to SW results in invalid manipulation, because of the smoothing step during distribution reconstruction. We thus study several attack variants, which report a value sampled in a range at the higher end, instead of always reporting the largest possible value. Experimental results demonstrate that SW and CFO under \textit{Server} setting provides better robustness than \textit{User} setting and consistently has lower \ASG/\SGR values. Furthermore, the \SGR value decreases as $\epsilon$ increases, approaching 1 for reasonable $\epsilon$ values. However, when $\epsilon$ is small (e.g. $0.1$), \SGR can be over 10 even for SW and CFO-based protocols under \textit{Server setting}, suggesting that the advanced attack can achieve over 10 times better performance than the baseline attack and that the data manipulation can be a serious concern in cases that demand high privacy.


% We also explore attack detection for the studied protocols. We find that the perturbed results in the CFO-based mechanisms only contain the information about which bins are supported. Thus, the only way to detect the presence of the attack is to observe unreasonably large frequencies of some bins given prior knowledge, which is challenging in practice. The SW mechanism, on the other hand, reports much richer information, as each report is a numerical value in a range. Therefore, we design an effective \textit{zero-shot attack detection} for SW by analyzing the distribution of reported values.

% \li{We also explore attack detection for the studied protocols and design an effective \textit{zero-shot attack detection} by analyzing the distribution of reported values. However, it is challenging to detect poisoning attack for CFO-based mechanisms under \textit{Server} setting and we find the existing defense since the attacker can only manipulate limited information that can be used for detection \cite{cao2021data}. Our detection is not the most accurate for CFO-based mechanisms under \textit{Server} setting.}

% \li{We also explore attack detection for the studied protocols. Existing defenses \cite{cao2021data} primarily focusing on CFO-based mechanisms exhibit poorly in practice. In particular, they either rely on knowledge about the true data distribution that is unknown to the server, or detect by only capturing unreasonably large frequencies of some bins. It fails to alert the attack when the number of the attacker-targeted bins is small (e.g., 1) since the statistical abnormality can be discerned if the frequency exceeds an high threshold and achieving this threshold demands compromising an exceptionally large number of users for attacker. Consequently, the feasibility of this detection method is deemed impractical. To address this problem, we design an effective \textit{zero-shot attack detection} by analyzing the distribution of reported values without any prior assumption.}

\li{We also explore attack detection for the studied protocols. Existing defenses \cite{cao2021data} primarily focusing on CFO-based mechanisms exhibit poorly in practice. In particular, they either rely on knowledge about the true data distribution that is unknown to the server, or by capturing unreasonably large frequencies of some bins. Solely using frequency information to detect is only effective when the attacker manipulates frequencies of a set of bins but fails when the number of the attacker-targeted bins is small (e.g., 1) since the statistical abnormality is not obvious in this case. To address this problem, we design an effective \textit{zero-shot attack detection} by analyzing the distribution of reported values without any prior assumption.}

The main idea of the detection is to leverage the distribution information to capture the difference between the randomness of fake values and the LDP perturbation. Specifically, we synthesize the data based on the distribution information and reconstruct two sets of noisy results by LDP perturbation. The group of pairwise distances between them can be used as the benchmark because they undergo the same LDP protocol and exhibit equivalent randomness. Next, we calculate a second group of distances between the reported result and the set of reconstructed results and statistically analyze the closeness between this distance group and the benchmark by the two-sample KS test, which is a hypothesis test method to determine if two groups of samples follow the same distribution. When these two distance groups are close, the reported results have similar randomness to the benchmark and thus are considered unpolluted. We plot the ROC curve and use the area under the curve (AUC) to evaluate the detection performance with multiple datasets. The larger AUC indicates a better result.
% The AUC of our detection constantly remains over 0.97 on all datasets in the presence of only $5\%$ malicious users. We also empirically analyze detection effectiveness against attack performance. The results show that when the attack evades detection, the attack efficacy also diminishes significantly, leading it close to the baseline, which means the attack is no longer a serious security concern.
\li{The experimental results show our detection performs much better than existing detection. Especially on SW, OUE and other CFO-based mechanisms under \textit{User} setting, the AUC constantly remains over 0.92 on all datasets in the presence of only $5\%$ malicious users. In the meanwhile, our detection also improve the limitation of existing detection on \textit{Server} setting. We also empirically analyze detection effectiveness against attack performance. The results show that when the attack evades detection, the attack efficacy also diminishes significantly, leading it close to the baseline, which means the attack is no longer a serious security concern.}
We summarize the contribution below.

\begin{enumerate}[leftmargin=*]
    % \item We propose distribution-shift-maximization data poisoning attacks against LDP protocols for numerical data. This is the first paper to comprehensively investigate the robustness of full-distribution reconstruction LDP protocols for numerical data under poisoning attack.

    % \item We perform a comprehensive investigation on the robustness of LDP protocols for numerical data under data poisoning attacks.

    \item We performed a comprehensive investigation on the robustness of LDP protocols for numerical data under data poisoning attacks. We studied two types of state-of-the-art LDP protocols: 1) CFO with binning and consistency and 2) distribution recovery.

    % \item \sun{contribution about attack design, difference between CFO and SW.}
    % \li{We studied effective data poisoning attack and the results conclude that different attack strategies are necessary for CFO-based protocols and SW to achieve effective distribution manipulation.}
    \item We studied effective attacks to manipulate the distribution estimation. Our analysis and experiment show that there is no ``one-size-fits-all'' strategy to attack different LDP protocols. 
    % \item We theoretically and empirically evaluate the attacks on two types of state-of-the-art LDP protocols for numerical values: 1) CFO with binning and consistency and 2) distribution recovery. Our experimental results show that \textit{Server} setting provides much better robustness than \textit{User} setting. Protocols under \textit{Server} setting and SW are the most robust mechanisms by nature against the proposed data poisoning attack.

    % \item \sun{Robustness insights}
    \item We theoretically and empirically evaluate and compare the robustness of the state-of-the-art LDP protocols. We found that not all protocols are equivalently resilient against the attack. CFO under \textit{Server setting} and SW offer better security.  
    
    \item We designed a new detection framework to identify data manipulation. Our method leverages the distribution properties of the reported data to detect attacks that introduce statistically significant bias to the distribution without knowing the ground truth information. The experiment confirmed the effectiveness of our detection in challenging scenarios. 
\end{enumerate}

% Specifically, we first estimate the data distribution from the noisy report and synthesize data follow this distribution. Given the synthetic data, we reconstruct two groups of noisy results by LDP perturbation and calculate a group of distances between them as benchmark since they are not polluted. Then we calculate a group of distances between the reported result and reconstructed results and statistically analyze the similarity between it with the benchmark distance group by KS test, which is a hypothesis test method to determine if the distributions of two groups of samples are similar. \sun{might need to be concise.} When these two distance groups are similar, the reported result is not polluted. We note that not all LDP mechanisms can return the distribution information and our framework cannot enhance security for such mechanisms. \sun{no need to mention here} For example, SR and PM only return a single value as estimate of mean. We evaluate the detection framework on multiple datasets and the results show the our detection can effectively capture the attack.


% In LDP context, users report data to the server.  All LDP protocols require the usage of some perturbation algorithm $\Psi(x): \mathcal{D} \rightarrow \hat{\mathcal{D}}$, where $\mathcal{D}$ is the domain of user's values, and $\hat{\mathcal{D}}$ is the output domain of $\Psi$.  A user with private value $x$ would report $\Psi(x)$.  
% Some of these users may be malicious or compromised by an attacker and intentionally report wrong results.  If a malicious user with private value $x$ reports $\Psi(x')$, then this behavior is indistinguishable from a user whose true value is $x'$.  This is considered the baseline of poisoning attacks.  However, malicious users can directly choose values in $\hat{\mathcal{D}}$ that best achieve the attack objective and report these carefully chosen values.  Different LDP protocols may have very different degrees of vulnerability to such attacks.  



% In this paper, we study the effect of poison attacks against LDP protocols for numerical data.  In the literature, Cheu \textit{et al.} \cite{cheu2021manipulation} studied \textit{untargeted attack} against frequency oracles in categorical data. Wu \textit{et al.} \cite{wu2021poisoning} and Cao \textit{et al.} \cite{cao2021data} studied \textit{targeted attacks} to maximally promote the associated statistics on attacker-chosen items or key-value data. \li{Different from maximizing the statistics, Li \textit{et al.} \cite{li2022fine} investigated the \textit{fine-grained attack} to simultaneously manipulate the mean and variance to target values.} \sun{include our fine-grained attacks? and discuss it related work as well} \li{To the best of our knowledge, we are the first to study poisoning attacks against LDP protocols for numerical data.} \sun{mean/variance are also numerical? and key value?} We aim to answer the following research questions:  (1) What are the most effective attacks against different LDP protocols? \sun{I think it is too broad}  (2) How different LDP protocols compare in terms of robustness against poisoning attacks?  Typically LDP protocols are compared based on estimation accuracy; robustness adds another interesting dimension one should consider when choosing a LDP protocol. \sun{what is the definition of robustness?}  (3) How to detect such poisoning attacks?

% \li{natural robustness and active detection.}

% For attack objective, we focus on increasing (or decreasing) estimated mean.  Mean estimation is the task that several protocols are specifically designed for, and can be used to estimate other statistical quantities, such as the variance.  
% To evaluate the effectiveness of a mean-manipulation attack, a natural metric is to measure the mean gain $| \hat{\mu}_a - \mu |$, where $\hat{\mu}_a$ is the estimated mean after attack. However, mean gain is influenced by factors such as the privacy parameter $\epsilon$ and the fraction of users that are assumed to be malicious; it does not directly yield the strength of an attack or the robustness of a LDP protocol.  We propose a new metric called mean gain ratio (MGR). The key intuition is to measure the ratio of the mean gain from the proposed attack, i.e., $| \hat{\mu}_a - \mu |$, to the mean gain of the baseline, i.e., $| \hat{\mu}_a^{base} - \mu |$. Due to the LDP noise, the mean gain of the baseline attack is random and attacks with the same $\hat{\mu}_a$ may have different measurement. Therefore, we substitute the term $\hat{\mu}_a^{base}$ with the skewed mean in the input domain since the estimated mean in a well-designed LDP protocol is unbiased and close to the mean in the input domain. By this substitution, the denominator of MGR is a constant.  An MGR value of $1$ means that the attack is no more effective than the baseline and should not be a concern.  On the other hand, a high MGR value, such as $10$ or higher, is highly concerning.  Thus, we can easily use MGR to compare different attacks as well as different LDP protocols. 

% We study four state-of-the-art LDP mechanisms for numerical data.  SR \cite{duchi2018minimax} and PM \cite{wang2019collecting} were designed for mean estimation.  CFOB \cite{li2020estimating} and SW \cite{li2020estimating} were designed to output a distribution, from which one can compute the mean.   In~\cite{li2020estimating}, it was demonstrated that SW can give more accurate estimates for mean and variance. 


% We formulate the attack as an optimization problem.  
% Moreover, we theoretically and empirically study the effectiveness of the attack. Theoretically, we find it is challenging to solve the optimal fake values for SW mechanism since the output of SW mechanism depends on distribution of the underlying true data and the attack efficacy is unpredictable to the attacker. \li{Prior work studied the relationship between the security of LDP protocols and privacy budget $\epsilon$ varies under different attacks. Specifically, under targeted attacks, recent works \cite{cheu2021manipulation, cao2021data} show the security-privacy tradeoff for LDP protocols: smaller $\epsilon$ provides higher privacy but weaker security. Under fine-grained attack \cite{li2022fine}, smaller $\epsilon$ provides stronger security because it leads to larger noise and greater error between estimated results and target values. This property is called security-privacy consistency. However, we find neither tradeoff nor consistency holds for SW mechanism, which further complicates the attack since it is challenging to determine when the security of SW is weak.}
% Empirically, we evaluate the attack on multiple datasets. Due to the lack of optimal attack, we intuitively inject four types of large values (or small values) to SW for increasing the mean (or decreasing the mean). The results show the best attack type varies under different datasets and $\epsilon$ and there is no optimal attack. Besides, the MGR of attack on SW is lower than other mechanisms in most cases, indicating SW can naturally resist the attack.



% Attack detection strategy is widely used to mitigate poisoning attacks. Generally, the defender uses information about genuine users or true data as the benchmark and determines if the attack occurs \cite{gong2014sybilbelief, jia2017random}. However, in LDP scenario, there is no benchmark. Trapped in this challenge, existing mitigations are not practical since they either rely on strong assumptions about the true data or only work well in worst cases \cite{cao2021data, wu2021poisoning}. To further enhance the LDP security, we also investigate the attack detection framework for LDP protocols for mean estimation. The key intuition is to leverage the distribution information returned by LDP protocols to construct the benchmark for detection. Specifically, we first estimate the data distribution from the noisy report and synthesize data follow this distribution. Given the synthetic data, we reconstruct two groups of noisy results by LDP perturbation and calculate a group of distances between them as benchmark since they are not polluted. Then we calculate a group of distances between the reported result and reconstructed results and statistically analyze the similarity between it with the benchmark distance group by KS test, which is a hypothesis test method to determine if the distributions of two groups of samples are similar. \sun{might need to be concise.} When these two distance groups are similar, the reported result is not polluted. We note that not all LDP mechanisms can return the distribution information and our framework cannot enhance security for such mechanisms. \sun{no need to mention here} For example, SR and PM only return a single value as estimate of mean. We evaluate the detection framework on multiple datasets and the results show the our detection can effectively capture the attack.


% We summarize the contribution below.
% \begin{enumerate}
%     \item We perform the first systematic study on optimal poisoning attack to LDP protocols for mean estimation, and analyze the robustness of a family of LDP mechanisms under the attack.
    
%     \item We propose a new metric for attack efficacy. This metric considers the baseline attack \sun{remind what is baseline} and can show how much the attack outperforms the baseline.
    
%     \item We design a new detection framework for poisoning attack. It can effectively detect the attack without knowing the ground truth.
    
%     \item We comprehensively evaluate the attack and the detection on three real-world datasets and one synthetic dataset. The empirical study shows SW mechanism can naturally resist the proposed attack, and the framework can effectively capture the attack.
% \end{enumerate}

==> 3_attack.tex <==
\section{Attacking LDP Protocols for Numerical Attributes} \label{sec:attack_model}
This section introduces our attack model, including the attacker's capability and the attack goal.
Then we introduce a metric for the distribution shift attack and attack details.

\subsection{Attack Model}
\noindent\textbf{Attacker's Capability.}
To be consistent with previous work \cite{cheu2021manipulation}, we assume the attacker can control a small proportion of the users to send crafted fake values to the server. 
Specifically, let the total number of users be $n$.
The attacker compromises $n_f = \beta n$ users $(0 \leq \beta \leq 1)$, who send fake values $\hat{Y} = [\hat{y}^{(i)}]_{i=1}^{n_f}$ to the server. 
The remaining $n_g = (1-\beta)n$ users are benign users sending the perturbed true values to the server.
We also assume the attacker can access the encoding and perturbation steps in the LDP protocol because these steps are deployed locally. Therefore, the attacker knows the parameters in the LDP protocols, including the privacy budget $\epsilon$, perturbation probability, and the number of bins.

\noindent\textbf{Attacker's Goal.}
The attacker aims to shift the distribution to the right-most end as much as possible.
% Since the estimated distribution is over a metric space, point-wise distance metric is not suitable.
% Therefore, we define the attacker's goal as to maximize the Wasserstein distance \cite{li2020estimating} \zl{new metric?} between the shifted distribution and the original distribution, which measures the overall similarity between two distributions.
% Shifting the distribution to the left-most end is analogous, which we do not consider in this paper.
% \li{Therefore we define two metrics to measure the degree of distribution shift towards right side (See Sectoin~\ref{sec:attack_effectiveness}).}
Shifting the distribution to the left-most end is a symmetric goal,  which we will not delve into due to space constraints.
% \vspace{3pt}

\noindent\textbf{Baseline Attack.}
In the general LDP context, the baseline attack on the LDP protocol is that the attacker skews the estimates by providing fake values in the input domain to the LDP protocol and reporting those randomized outputs. It can be understood as one of the special kinds of \emph{input manipulation} as in \cite{cheu2021manipulation, li2022fine}. For distribution-shift attacks, since the frequencies of all bins sum up to one, an effective way to shift the distribution is to maximally increase the frequency of the right-most bin and decrease the frequencies of other bins in the meanwhile. Therefore, the baseline attacker injects maximums in the input domain of the LDP protocol as fake values. 
Specifically, the baseline attacker repeats $\Psi_{\mathrm{HST}}(m_o)$ (or correspondingly, $\Psi_{\mathrm{OLH}}(m_o)$ for OLH, $\Psi_{\mathrm{SW}}(1)$ for SW) for $n_f$ times and sends the randomized outputs to the server.

% \zl{move this to after the first sentence of previous paragraph, to serve as the reason for choosing such baseline?} \li{maybe we can discuss, I mentioned baseline is a special kind of input attack and I think this is a reason, and I want this paragraph to focus on explaining the property of baseline.} 
The users controlled by a baseline attacker behave identically to those users who happen to own and submit the same values by following the protocol. Therefore, without prior information about the true distribution or other authentication techniques, the server has no way to detect the baseline attack.
Due to the unbiasedness of LDP protocols, the aggregated distribution (before consistency) of the baseline attack $\hat{X}_{a}^{base}$ is approximately equal to $\mathbb{E}(\hat{X}_{a}^{base}) = X_a^{base}$, where $X_a^{base}$ is the skewed distribution in the input domain after baseline attack. Therefore, the outcome of baseline attack is almost independent of post-processing since $X_a^{base}$ has satisfied consistency.
% The outcomes of the baseline attacks are approximately equal to $\frac{1}{n}(\sum_{i=1}^{n_g}x_i + \sum_{j=1}^{n_f}y_i)$, where $y_i$ is the fake value sent from the $i$-th malicious user.
% In this paper, we investigate the attacks that can amplify the attack effect, which in turn are more susceptible to detection.



\subsection{Attack Effectiveness} \label{sec:attack_effectiveness}
To quantitatively measure the efficacy of the attacks, we use two metrics in this paper to show how far the poisoned distribution can deviate from the true distribution.

\noindent\textbf{Absolute Shift Gain (\ASG).}
\begin{figure}
    \centering
    \includegraphics[scale = 0.3]{version_2_NDSS_2023/figure/metric_intuition.pdf}
    \caption{Examples of \ASG. The difference between the cumulative functions of the original and shifted distributions is positive in the green area and negative in the red area.}
    \label{fig:metric_intuition}
    \vspace{-10pt}
\end{figure}
% \zl{need to clean up the content and make it consistent with the introduction.
% The attacker's goal is to maximally increase the estimated mean. Specifically, assume the true mean is $\mu$ and the estimated mean after the attack is $\hat{\mu}_a$. We define the mean gain as $\Delta_{\hat{\mu}_a} = \hat{\mu}_a - \mu$ and larger mean gain indicates more successful attack. 
% Because of the inherent randomness of the LDP protocols, the mean gain is also a random variable.
% Thus, we consider the overall mean gain using the expected gain as $G^+(\hat{\mu}_a) = \mathbb{E}(\Delta^{+}_{\hat{\mu}_a})$ and $G^-(\hat{\mu}_a) = \mathbb{E}(\Delta^{-}_{\hat{\mu}_a})$.
% With such definitions, the attacker aims to maximize the overall gain $G^+(\hat{\mu}_a)$ or $G^-(\hat{\mu}_a)$ to maximally increase or decrease the mean. Formally, the attacker aims to solve the following optimization problem:
% \begin{equation*}
%     \begin{aligned}
%         \underset{\hat{Y}}{\max} && G^+(\hat{\mu}_a), && \mathrm{increase~mean} \\
%         \underset{\hat{Y}}{\max} && G^-(\hat{\mu}_a), && \mathrm{decrease~mean}
%     \end{aligned}
% \end{equation*}
% A straightforward metric for attack efficacy is to measure \ASG by Wasserstein distance $W_1$, that is how much the attack shifts the estimated distribution. Denote the original and the estimated distribution as $X = [\Phi(B_i)]_{i=1}^{m_o}$ and $\hat{X}_a = [\Phi(\hat{B}_i)]_{i=1}^{m_o}$ respectively, the \ASG can be formally defined below,
% \begin{align*}
%     \ASG(\hat{X}_a) = W_1(X, \hat{X}_a) = \sum_{v=1}^{m_o} \left| P(X, v) - P(\hat{X}_a, v) \right|,
% \end{align*}
% where $P(X, v) = \sum_{i=1}^{v} \Phi(B_i)$ is the cumulative function over distribution $X$. Larger \ASG indicates larger distance between $X$ and $\hat{X}_a$ and better attack efficacy.
A straightforward metric for attack efficacy is Wasserstein distance, which measures the distance between the estimated distribution with the poisoning attack and the clean one. 
However, it cannot reflect the direction in which the attacked distribution is skewed.
Any local skews on the distribution, whether towards the right or left, can increase the Wasserstein distance.
% and directly using it could not correctly measure the extend to which the distribution is shifted to the right end since the distance could be the same if the distribution is shifted to the left.
To address this problem, we adapt the definition of $L_1$ Wasserstein distance but replace the $L_1$ norm with differences with signs to form our new metric. 
Denote the original and the estimated distribution as $X = [\Phi(B_i)]_{i=1}^{m_o}$ and $\hat{X}_a = [\Phi(\hat{B}_i)]_{i=1}^{m_o}$ respectively, the \ASG can be formally defined below,
% \begin{align*}
%     \ASG(\hat{X}_a) = W_1(X, \hat{X}_a) = \sum_{v=1}^{m_o} P(X, v) - P(\hat{X}_a, v),
% \end{align*}
\begin{align*}
    \ASG(\hat{X}_a) = \sum_{v=1}^{m_o} P(X, v) - P(\hat{X}_a, v),
\end{align*}
where $P(X, v) = \sum_{i=1}^{v} \Phi(B_i)$ is the cumulative function over distribution $X$. The intuition behind the metric is shown in Figure~\ref{fig:metric_intuition}. As the distribution is shifted to the right end, the value of the cumulative function on the left side of the domain is getting smaller while becomes larger on the right side. The farther the distribution is shifted to the right end, the larger $\sum_{v=1}^{m_o} P(X, v)$ is than $\sum_{v=1}^{m_o} P(\hat{X}_a, v)$. Thus, larger \ASG indicates a better shift effect and better attack efficacy. Besides, negative \ASG indicates the overall distribution is shifted to the left side.


\noindent\textbf{Shift Gain Ratio (\SGR).}
The \ASG is a straightforward metric that aligns with the attacker's goal and can measure the ultimate effectiveness of all kinds of attacks on the numerical LDP protocols.
However, it is implicitly influenced by many factors, including how many users are corrupted by the attacker and what the true data distribution is.
Besides, as we look into the attacks that are more effective than the baseline attacks, \ASG fails to demonstrate the advantage of those attacks over the baseline attacks.
Thus, we propose a new metric, \SGR, to measure the effectiveness of the proposed attacks compared to the baselines and thus enable the analysis of the robustness of LDP protocols.
% In this paper, we propose a new metric to measure the poisoning attack efficacy. 
% \li{A straightforward metric is to measure the \textit{mean gain} for each attack, i.e., $\Delta^{+}_{\hat{\mu}_a}$ (or $\Delta^{-}_{\hat{\mu}_a}$) for increasing (or decrease) the mean.} 
% However, this metric does not evaluate how much the attack outperforms the baseline attack. 


% To address this problem, we consider the ratio of the mean gain from advanced attack to that of the baseline attack. 
We first consider the ratio of the shift gain of our attack to that of the baseline attack, i.e., $\frac{\ASG(X, \hat{X}_{a})}{\ASG(X, \hat{X}_{a}^{base})}$,
% Specifically, the mean gain ratio (MGR) of skewed mean $\hat{\mu}_a$ is
% \begin{align*}
%     MGR(\hat{\mu}_a) = \frac{\hat{\mu}_{a} - \mu}{\hat{\mu}_{a}^{base} - \mu},
% \end{align*}
where $\hat{X}_{a}^{base}$ is the estimated distribution after baseline attack. However, directly using this ratio as a metric may lead to an unstable measurement of additional variance because the denominator includes $\hat{X}_{a}^{base}$, a random variable with LDP noise.
% and even two attacks have the same $\hat{\mu}_a$, this ratio shows different measurement. 
%On the other hand, any valuable LDP protocols that can be used to estimate the mean should give an unbiased and stable mean estimate.
We replace the term $\hat{X}_{a}^{base}$ with the skewed distribution in the input domain $X_{a}^{base}$. %\zl{definition missing?}
Note that this is a reasonable substitution because the estimated distribution in well-designed LDP protocols should be close to the distribution in the input domain. Formally, 
\begin{align}
    \SGR(\hat{X}_a) = \frac{\ASG(X, \hat{X}_{a})}{\ASG(X, X_{a}^{base})}
    \label{eq:proposed_attack_metric}
\end{align}

% \zl{I tried remove all $W_1$ in the introduction of \ASG and \SGR, because they are not wasserstein.}
By Equation \eqref{eq:proposed_attack_metric}, a smaller value of the metric means lower attack efficacy. Specifically, the metric equal to 1 indicates the attack performs similarly to the baseline. When the metric is less than 1, the attack underperforms the baseline. Moreover, when the ratio is negative, the attack efficacy tends to move in a different direction than the baseline, e.g., the baseline shifts the distribution to the right end, but the measured attack is not able to achieve this goal.

With a predetermined dataset and a fixed number of corrupted users, \SGR is proportional to \ASG. However, the normalization with the baseline attack gain brings two benefits. The first is that \SGR is more consistent for the protocols across different datasets.
Another is that \SGR can show how the attack efficacy is affected by different portions of corrupted users, while the \ASG will monotonically increase with the corrupted portion.

% There is an important property of \SGR. Since the denominator is constant given $\beta$, the \SGR can also reflect the \ASG. In particular, the attack with larger ratio also has larger \ASG under the same $\beta$.

% It is worth noting that the metric has two properties below.
% \begin{enumerate}
%     \item The metric measures the ratio between attack gains, which is essentially how much each compromised user can improve the baseline attack. Therefore, it is independent of the number of malicious users. \zl{It may be not that clear as a direct property. Maybe as a conclusion of the experimental results?}
    
%     \item The denominator of the metric is constant given $\beta$. Thus, the metric can also reflect the attack gain. In particular, the attack with larger ratio also has larger attack gain under the same $\beta$.
% \end{enumerate}


% \subsection{Attacks on Mean Estimation Protocols}
\subsection{Attacks on CFO with binning and consistency}


% For a valid distribution estimate, the frequencies of all bins sum up to one due to the consistency.
% Therefore, an effective way to shift the distribution to the right-most end is to promote the frequencies of large values in the right side of the domain and accordingly reduce the frequencies of other bins.
% Following this logic, we study how to attack OUE, HST and OLH. The main idea of our attack is to increase the frequency of the largest value as much as possible.
% We note that there may exist more effective attack and can achieve the better attack efficacy. However, the basic intuition is similar to ours. Additionally, our research goal is to study and compare the robustness of LDP protocols under different settings. Thus, the sub-optimal attack does not affect the main conclusion in this paper.

Optimal attacks for shifting distribution with different FO depend on the real data distribution, which may not be known to the attacker in general. However, the main idea of shifting the distribution to the right side is to increase the frequencies of large values. For robustness analysis, we consider a straightforward heuristic attack that increases the frequency of the largest value $\Phi(B_{m_o})$ as much as possible. This attack can ensure the distribution is shifted in the direction as attacker expected for all distribution and empirically achieves significant attack efficacy. We elaborate on $\Phi(B_{m_o})$ with $n_f$ malicious users and the creation of fake report to each protocol.

\mypara{Attacking OUE.} The aggregated result $\Phi(B_{m_o})$ and corresponding fake reports are as follows.
\begin{itemize}
    \item \textbf{Aggregation $\Phi(B_{m_o})$:} The estimated frequency $\Phi(B_{m_o}) = \frac{\sum_{j=1}^{n_g} \hat{\bm{v}}^{(j)}[m_o] + \sum_{j=1}^{n_f} \hat{\bm{y}}^{(j)}[m_o] - \frac{n}{e^\epsilon + 1}}{\frac{1}{2} - \frac{1}{e^\epsilon + 1}}$.

    \item \textbf{Fake report craft:} Since the compromised users in OUE are able to craft the fake report vector $\hat{\bm{y}}$, the most effective way to promote $\Phi(B_{m_o})$ is to craft $\hat{\bm{y}} = [0, 0, .., 1]$ such that only the frequency of the $m_o$-th bin is contributed.
\end{itemize}
% Under the attack, the estimated frequency of the $m_o$-th bin is $\Phi(B_{m_o}) = \frac{\sum_{j=1}^{n_g} \hat{\bm{v}}^{(j)}[m_o] + \sum_{j=1}^{n_f} \hat{\bm{y}}^{(j)}[m_o] - \frac{n}{e^\epsilon + 1}}{\frac{1}{2} - \frac{1}{e^\epsilon + 1}}$.
% Since the compromised users in OUE are able to craft the fake report vector $\hat{\bm{y}}$, the most effective way to promote $\Phi(B_{m_o})$ is to craft $\hat{\bm{y}} = [0, 0, .., 1]$ such that only the frequency of the $m_o$-th bin is contributed.

\mypara{Attacking HST.}
There are two different implementations of HST depending on whether users or the server samples the public vector $s^{(i)} \in \{\pm 1\}^{m_o}$. Without the attack, these two implementations give the same privacy and utility guarantee.
However, our experiments show that when the server generates the public vector for each user, the attack can be largely constrained on his attack efficacy.
% Meanwhile, although post-processing methods for consistency can ensure the output to be a valid distribution, there is no closed-form solution for the expectation of normalized frequencies after applying it. \zl{is this the problem with all CFO?}
Thus, we elaborate on our two implementations as follows.

\mysubpara{HST-User.}
% When the users are able to select public vectors by themselves, they can pick binary vectors that promote the frequency of the largest value in the domain. Thus, the estimated frequency of the $m_o$-th bin is $\Phi_{\mathrm{HST}}(B_{m_o}) = \frac{1}{n} (\sum_{j=1}^{n_g} \hat{s}^{(j)}_{x_b} \times \bm{s}^{(j)}[m_o] + \sum_{j=1}^{n_f} \hat{y}^{(j)} \times \hat{\bm{s}}^{(j)}[m_o])$ under the attack, where $\hat{\bm{s}}^{(j)}$ is the binary vector picked by malicious user $j$. 
% The idea of promoting $\Phi(B_{m_o})$ is to craft fake value $\hat{y}^{(j)}$ and carefully select public binary vector $\hat{\bm{s}}^{(j)}$ so that the aggregated result $\hat{y}^{(j)} \times \hat{\bm{s}}^{(j)}[m_o]$ only contributes to $\Phi_{HST}(B_{m_o})$. Specifically, the attacker sets the public binary vector as $s^{(i)} = [-1, -1, ..., 1]$ where only the largest bin is 1, and then crafts fake value $\hat{y}_i$ as $\frac{e^\epsilon + 1}{e^\epsilon - 1}$ to maximally increase the frequency of the largest value.
The aggregated result $\Phi(B_{m_o})$ and corresponding fake reports are as follows.
\begin{itemize}
    \item \textbf{Aggregation $\Phi(B_{m_o})$:} When the users are able to select public vectors by themselves, they can pick binary vectors that promote the frequency of the largest value in the domain. Thus, the estimated frequency of the $m_o$-th bin is $\Phi_{\mathrm{HST}}(B_{m_o}) = \frac{1}{n} (\sum_{j=1}^{n_g} \hat{s}^{(j)}_{x_b} \times \bm{s}^{(j)}[m_o] + \sum_{j=1}^{n_f} \hat{y}^{(j)} \times \hat{\bm{s}}^{(j)}[m_o])$, where $\hat{\bm{s}}^{(j)}$ is the binary vector picked by malicious user $j$.

    \item \textbf{Fake report craft:} The idea of promoting $\Phi(B_{m_o})$ is to craft fake value $\hat{y}^{(j)}$ and carefully select public binary vector $\hat{\bm{s}}^{(j)}$ so that the aggregated result $\hat{y}^{(j)} \times \hat{\bm{s}}^{(j)}[m_o]$ only contributes to $\Phi_{HST}(B_{m_o})$. Specifically, the attacker sets the public binary vector as $\bm{s}^{(j)} = [-1, -1, ..., 1]$ where only the largest bin is 1, and then crafts fake value $\hat{y}^{(j)}$ as $\frac{e^\epsilon + 1}{e^\epsilon - 1}$ to maximally increase the frequency of the largest value.
\end{itemize}

\mysubpara{HST-Server.}
% Unlike the previous implementation, the server set the public binary vector for each user uniformly at random at the beginning of the protocol. 
% Each user must use the assigned binary vector.
% Because the privacy guarantee is only based on randomization of the picked $s^{(i)}_{x_b}$ value but independent of the choice of $s^{(i)}$, this implementation provides the same level of privacy as HST-User.
% The attacker is constrained to use $s^{(i)}$ for its corrupted user $i$.
% Thus, it can only manipulate the fake value $\hat{y}_{i}$ as the same value as $\frac{e^\epsilon + 1}{e^\epsilon - 1} \times s^{(i)}_{m_o}$ and in this way the aggregated result $\hat{y}_i \times s^{(i)}_{m_o}$ can promote the largest value in the domain. 
% However, since the vector follows uniform distribution and each report supports about half of the bins, the attacker cannot only increase the frequency of the largest bin.
Unlike the previous implementation, the server set the public binary vector for each user uniformly at random at the beginning of the protocol. Thus, the aggregated result $\Phi(B_{m_o})$ and corresponding fake reports for HST-Server are different from HST-User.
\begin{itemize}
    \item \textbf{Aggregation $\Phi(B_{m_o})$:} Each user in HST-Server must use the assigned binary vector. Thus, the attacker is constrained to use $\bm{s}^{(j)}$ for its corrupted user $j$. Consequently, the estimated frequency of the $m_o$-th bin is $\Phi_{\mathrm{HST}}(B_{m_o}) = \frac{1}{n} (\sum_{j=1}^{n_g} \hat{s}^{(j)}_{x_b} \times \bm{s}^{(j)}[m_o] + \sum_{j=1}^{n_f} \hat{y}^{(j)} \times \bm{s}^{(j)}[m_o])$.

    \item \textbf{Fake report craft:} Attacker can only manipulate the fake value $\hat{y}^{(j)}$ as the same value as $\frac{e^\epsilon + 1}{e^\epsilon - 1} \times s^{(j)}[m_o]$ and in this way the aggregated result $\hat{y}^{(j)} \times \bm{s}^{(j)}[m_o]$ can promote the largest value in the domain. However, since the vector follows uniform distribution and each report supports about half of the bins, the attacker cannot only increase the frequency of the largest bin.
\end{itemize}


\mypara{Attacking OLH.}
Similar to HST, there are also two implementations for OLH depending on whether users or the server chooses the hash function, which is equivalent from the perspective of privacy and utility guarantee absent of the attack.
Given a hash function $H$, the attacker can search the hash mappings and learn the inverse of the hash function $H^{-1}$, mapping a hash output in $[g]$ to a subset of $[m_o]$.
Our experiments also show that when the server decides the hash functions for each user, the attacker can be largely constrained on its manipulation efficacy. 
We elaborate on our two implementations as follows.

\mysubpara{OLH-User.}
% When the users need to randomly choose the hash function by themselves, the attacker can choose the hash functions from a set of all hash functions $\mathbf{H}$ for the compromised users and promote the frequencies of largest values in the domain.
% To this end, the fake report $\langle \hat{H}, \hat{y}_h \rangle$ should satisfy two conditions: 1) $\hat{H}(m_o) = \hat{y}_h$ and 2) the size of the set of values that hashed into $\hat{y}_h$ by $\hat{H}$ is as small as possible.
% Ideally, the size is 1 and $\hat{H}$ can only hashes the largest value into $\hat{y}_h$. Such fake report can only increase the frequency of the $m_o$-th bin and maximally shift the distribution.
% However, we may be unable to find such $\langle \hat{H}, \hat{y}_h \rangle$ within a given amount of time in a large set $\mathbf{H}$.
% In our experiments, for each fake user, we randomly sample 1,000 hash functions as the hash function candidate set $\mathbf{H}$ to find the fake report satisfying the above conditions.
% When the users need to randomly choose the hash function by themselves, the attacker can choose the hash functions from a set of all hash functions $\mathbf{H}$ for the compromised users. Ideally, we hope to craft a fake report $\langle \hat{H}, \hat{y}_h \rangle$ where the hash function only maps the largest value into $\hat{y}_h$. However, we may not be able to find such a function within a given amount of time in the set $\mathbf{H}$. To address this problem, we randomly sample 1000 hash functions as the hash function candidate set in which we find the $\hat{H}$. The fake report should satisfy two conditions: 1) $\hat{H}(m_o) = \hat{y}_h$ and 2) all values mapped into $\hat{y}_h$ should concentrate on the higher end as much as possible, i.e., the mean of these values should be largest among all hash functions in $\mathbf{H}$. The first condition guarantees the fake report can promote the frequency of the largest value and the second condition guarantees the fake report would not contribute to frequencies of small values and impair attack efficacy.
The aggregated result $\Phi(B_{m_o})$ and corresponding fake reports are as follows.
\begin{itemize}
    \item \textbf{Aggregation $\Phi(B_{m_o})$:} When the users need to randomly choose the hash function by themselves, the attacker can choose the hash functions from a set of all hash functions $\mathbf{H}$ for the compromised users. Thus, the aggregated result $\Phi(B_{m_o}) = \frac{C_{g}(B_{m_o}) + C_{f}(B_{m_o}) - \frac{n}{g}}{n(\frac{e^\epsilon}{e^\epsilon + g - 1} - \frac{1}{g})}$, where $C_{g}(B_{m_o}) = |\{ j | H^{(j)}(m_o) = \hat{x}_h^{(j)}, j \in \mathrm{genuine\,users} \}|$, $C_{f}(B_{m_o}) = |\{ j | \hat{H}^{(j)}(m_o) = \hat{y}^{(j)}, j \in \mathrm{malicious\,users} \}|$ and $\langle \hat{H}^{(j)}, \hat{y}^{(j)} \rangle$ is fake report of malicious user $j$.

    \item \textbf{Fake report craft:} Ideally, we hope to craft a fake report $\langle \hat{H}^{(j)}, \hat{y}^{(j)} \rangle$ where the hash function only maps the largest value into $\hat{y}^{(j)}$. However, we may not be able to find such a function within a given amount of time in the set $\mathbf{H}$. To address this problem, we randomly sample 1000 hash functions as the hash function candidate set in which we find each $\hat{H}^{(j)}$. The fake report should satisfy two conditions: 1) $\hat{H}^{(j)}(m_o) = \hat{y}^{(j)}$ and 2) all values mapped into $\hat{y}^{(j)}$ should concentrate on the higher end as much as possible, i.e., the mean of these values should be largest among all hash functions in $\mathbf{H}$. The first condition guarantees the fake report can promote the frequency of the largest value and the second condition guarantees the fake report would not contribute to frequencies of small values and impair attack efficacy.
\end{itemize}

\vspace{-5pt}
\mysubpara{OLH-Server.}
% Unlike the previous implementation, the server picks a hash function for each user at the beginning of the protocol. 
% Each user must use the assigned hash function to hash the input.
% Because the privacy guarantee is only based on randomization after the hashed value, this implementation provides the same level of privacy as OLH-User.
%% The fake report should still satisfy the two conditions as OLH-User, but the attacker is constrained to use hash function $H^{(j)}$ for its corrupted user $j$.
% Thus, the attacker can only manipulate $\hat{y}_j$ to achieve the conditions.
% The attacker is constrained to use the assigned hash function for its corrupted user. Thus, the the attacker only needs to find $\hat{y}_j$ such that $H^{(j)}(m_o) = \hat{y}_j$.
OLH-Server has different aggregated result $\Phi(B_{m_o})$ and corresponding fake reports since the server picks a hash function for each user at the beginning of the protocol.
\begin{itemize}
    \item \textbf{Aggregation $\Phi(B_{m_o})$:} Since all users are constrained to use the assigned hash functions, the aggregated result $\Phi(B_{m_o}) = \frac{C_{g}(B_{m_o}) + C_{f}(B_{m_o}) - \frac{n}{g}}{n(\frac{e^\epsilon}{e^\epsilon + g - 1} - \frac{1}{g})}$, where $C_{g}(B_{m_o})$ is the same as that in OLH-User but $C_{f}(B_{m_o}) = |\{ j | H^{(j)}(m_o) = \hat{y}^{(j)}, j \in \mathrm{malicious\,users} \}|$ and $\langle H^{(j)}, \hat{y}^{(j)} \rangle$ is fake report of malicious user $j$.

    \item \textbf{Fake report craft:} The attacker is constrained to use the assigned $H^{(j)}$ for its corrupted user. Thus, the the attacker only needs to find $\hat{y}^{(j)}$ such that $H^{(j)}(m_o) = \hat{y}^{(j)}$.
\end{itemize}

\mypara{Theoretical Analysis.} \label{sec:theoretical_analysis}
% The relationship between LDP privacy and its vulnerability to data poisoning attacks is complex and depends on many factors \cite{li2022fine}. Prior work shows that there exists a tradeoff between security and privacy for LDP frequency estimation under poisoning attacks \cite{cao2021data, wu2021poisoning}. Informally, when the privacy budget $\epsilon$ is smaller, the frequency gain is larger. This is because the estimated frequencies are scaled up by a larger factor under smaller $\epsilon$. To further explore the vulnerability of LDP protocols to data poisoning attacks, we focus on other factors and study the relationship between security and the size of the hash domain $g$ for local hashing-based CFOs (e.g., OLH and HST). It is challenging to solve the exact attack efficacy given $g$ since the post-processing methods have no closed-form solution. Therefore, we establish the relationship between attack efficacy and $g$ without post-processing.
Prior work shows there is an inherent security-privacy tradeoff for frequency estimation protocols (the building block of CFO with binning and consistency) under frequency-maximization attack \cite{cao2021data, wu2021poisoning}. Informally, when the privacy budget $\epsilon$ is smaller, the frequency gain is larger. This is because the estimated frequencies are scaled up by a larger factor under smaller $\epsilon$. To further explore the vulnerability of LDP protocols to data poisoning attacks, we focus on other factors and study the relationship between security and the size of the hash domain $g$ for local hashing-based CFOs (e.g., OLH and HST). It is challenging to solve the exact attack efficacy given $g$ since the post-processing methods have no closed-form solution. Therefore, we establish the relationship between attack efficacy and $g$ without post-processing, shedding light on their relationship after post-processing, although consistency is not considered. 
% \sun{Is this a duplicate?}

\begin{theorem}
    % For local hashing based CFOs (e.g., HST and OLH) with fixed $\epsilon$, when the hash domain $g$ is smaller (large), our attack achieves a lower (higher) shift gain before post-processing for consistency.
    For local hashing based CFOs (e.g., HST and OLH) with fixed $\epsilon$, the expected \ASG/\SGR is proportional to $\frac{1}{g}$. When the hash domain $g$ is smaller (large), our attack achieves a lower (higher) shift gain before post-processing.
    \label{the:security_g_relationship}
\end{theorem}
\begin{proof}
    See Appendix~\ref{app:proof_security_g_relationship}
\end{proof}
% There is an intuition behind Theorem~\ref{the:security_g_relationship}. In the aggregation, each report can contribute to the frequencies of $\frac{m_o}{g}$ bins in average, which is getting less as $g$ grows. Therefore, it is easier for compromised users to contribute only the large values with large $g$, leading to better attack performance.

% Although Theorem~\ref{the:security_g_relationship} does not consider consistency, it sheds light on the relationship between attack efficacy and $g$ after post-processing.
There is an underlying intuition. In the aggregation, each report can contribute to the frequencies of $\frac{m_o}{g}$ bins in average, which is getting less as $g$ grows. Consequently, it is easier for compromised users to contribute only to the bins associated with large values when $g$ is larger, leading to enhanced attack performance. We also empirically study it and confirm it by our experiments (see Section~\ref{sec:security_g_relationship}), which demonstrates a correlation between increased $g$ and weakened LDP security.

\begin{figure*}
    \centering
    \includegraphics[scale = 0.33]{../figure/data_dist.pdf}
    \caption{Datasets Distribution}
    \label{fig:data_dist}
\end{figure*}

\subsection{Attacks on SW}
% As introduced in Section \ref{sec:background}, the expected value of mean for OLHB and SW have the similar form 
% \begin{align}
%     \mathbb{E}\left[ \sum_{i=1}^{m} h_i \times v_{B_i} \right].
%     \label{eq:expected_mean_OLHB_SW}
% \end{align}
% Thus, we study how to maximize Equation~\ref{eq:expected_mean_OLHB_SW} for OLHB and SW.

% According to Section~\ref{sec:background}, the expected value of mean for SW is 
% \begin{align*}
%     \mathbb{E}\left[ \sum_{i=1}^{m_s} h_i \times v_{B_i} \right].
% \end{align*}
% \begin{align*}
%     G(\hat{\mu}_a) = \mathbb{E}\left[ \sum_{i=1}^{m_s} h_i \times v_{B_i} - \mu \right].
% \end{align*}
% Following the same logic, the solution to shift the distribution under SW is still promoting the frequency of the large values in the domain while accordingly reducing other values frequencies.
% However, the convergence point of EMS algorithm depends on the privacy budget $\epsilon$ and the underlying data which is unknown to the attacker \cite{li2020estimating}. Therefore, the recovered distribution $[h_1, ..., h_m]$ is unpredictable to the attacker. As thus, it is challenging for the attacker to find the optimal fake values in theory. Injecting only the maximum values can lead to invalid input for the EMS algorithm.

% To reconcile the theoretical gap, we consider an intuitive way to achieve the attack in practice. We injects the fake values into the bins near the right end of the output domain $[-b, 1+b]$ to promote the frequencies of large values. Specifically, we inject fake values in four ways. We uniformly at random inject the fake values into 1) the right-most bin, 2) range $[1+\frac{2b}{3}, 1+b]$, 3) range $[1, 1+b]$ and 4) range $[1-b, 1+b]$.

The convergence point of EMS algorithm depends on the privacy budget $\epsilon$ and the underlying data which is unknown to the attacker \cite{li2020estimating}. Consequently, the recovered distribution is unpredictable to the attacker and it is also challenging to find the optimal attack for SW. Following the same logic as the attack to CFO with binning and consistency, the solution to shift the distribution under SW is still promoting the frequencies of the large values in the domain while accordingly reducing other values frequencies.

We consider an intuitive way to achieve the attack in practice. We injects the fake values into the bins near the right end of the output domain $[-b, 1+b]$ to promote the frequencies of large values. Specifically, we inject fake values in four ways. We uniformly at random inject the fake values into 1) the right-most bin, 2) range $[1+\frac{2b}{3}, 1+b]$, 3) range $[1, 1+b]$ and 4) range $[1-b, 1+b]$.

% \vspace{3pt}




% There is an intuition behind Theorem~\ref{the:security_privacy_tradeoff}. For SR, the aggregated result is scaled by a parameter to obtain the unbiased mean estimate. The parameter is related to $\epsilon$ and a smaller $\epsilon$ makes the aggregated result scale up further. However, since the fake values are independent of $\epsilon$, smaller $\epsilon$ makes the fake values contribute more towards the estimated mean, leading to higher attack efficacy. Although PM does not scale the aggregated result, the fake values rely on $\epsilon$. A small $\epsilon$ expands the output domain of PM and the fake values may become larger. Thus, the estimated mean is skewed more and the attack efficacy is higher under a smaller $\epsilon$.

% It is challenging to theoretically verify the security-privacy tradeoff for OLHB and SW since there is no definite expression of the optimal solution of fake values. However, the empirical study in Section~\ref{sec:attack_experiments} shows that the attack efficacy is also close to the baseline as $\epsilon$ grows.

==> mitigation_experiment.tex <==
\section{Mitigation Evaluation}

\subsection{Setup}
\noindent\textbf{Datasets.}
We use the same datasets as attack evaluation introduced in Section~\ref{sec:attack_experiments}.

\noindent\textbf{Metric.}
The proposed mitigation classifies the reported result as ``polluted" or ``not polluted". Therefore, we can use metric for binary classifier to measure the performance of our mitigation. Receiver operating characteristic (ROC) curve \cite{fawcett2006introduction} is a widely-used method to illustrate the diagnostic ability of a binary classifier. It captures the relationship between true positive rate and false positive rate of the classifier. The larger the area under the curve (AUC), the better the classifier performs. We run each attack 50 times and plot the ROC curve for our countermeasure and measure the AUC as the metric for mitigation performance.

\noindent\textbf{Parameter Settings.}
Our mitigation depends on the number of perturbation times $m$ and the significance level $\alpha$. We set the default $m = 10$. For a low probability of type \uppercase\expandafter{\romannumeral1} error occurring, we set default $\alpha = 0.002$. According to the theoretical and empirical analysis, there is a security-privacy tradeoff for LDP protocols and the attack efficacy reduces as $\epsilon$ grows. Therefore, we evaluate the mitigation under small $\epsilon$. Specifically, we set $\epsilon = 0.2$, 0.6 and 1. In order to be consistent with parameter setting in attack evaluation, we still set $\beta = 5\%$, $7.5\%$ and $10\%$, $m_c = 32$ and $m_s = 512$.



\subsection{Results}

\subsubsection{ROC of Mitigation}

\begin{figure*}
    \centering
    \includegraphics[scale = 0.35]{../figure/ROC_eps_m5.pdf}
    \caption{ROC curve of proposed mitigation under $\beta = 5\%$ with varying $\epsilon$.}
    \label{fig:roc_eps_m5}
\end{figure*}

% We observe similar ROC curves when the attacker's goal is to increase or decrease the mean under $\beta = 5\%$, $7.5\%$ and $10\%$. Here we only elaborate on increasing the mean under $\beta = 5\%$ in Figure~\ref{fig:roc_eps_m5} and leave the detail about other ROC curves in Figure~\ref{} in Appendix~\ref{app:supplemental_experiment_results}.

We observe similar ROC curves when the attacker's goal is to increase or decrease the mean. Here we only elaborate on increasing the mean in Figure~\ref{fig:roc_eps_m5} and leave the detail about other ROC curves in Figure~\ref{} in Appendix~\ref{app:supplemental_experiment_results}.

Overall, the results show our detection is effective and all AUC are larger than 0.97. Moreover, the detection performance reduces as $\epsilon$ grows. This is because larger $\epsilon$ results in smaller noise, and the distance between the reported bogus data and the reconstructed data is closer to the distance benchmark. The detection is also impacted by attack range. The AUC on attack range $[1-b, 1+b]$ is slightly lower than other attack ranges. This is because the fake values are uniformly injected into attack range, and comparing with other attack range, the distribution of fake values in $[1-b, 1+b]$ is closer to the output probability distribution of SW. The detection effectiveness also increases as $\beta$ grows, since more compromised users inject more fake values and makes the reported results more abnormal.


\subsubsection{Relationship between Main Gain and P-value}

\begin{figure*}
    \centering
    \includegraphics{}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}

Another interesting questions are, when does the mitigation not detect the attack well? In this case, how does the attack perform? To answer these questions, we study the relationship between the mean gain of the attack and the p-value in the detection. We vary $\epsilon$ and $\beta$ and select the best attack range (the mean gain is highest) under each parameter setting. By repeating the attack 10 times, we use scatterplot to show the mean gain distribution as the function of p-value in detection. We only show the results when the attacker's goal is to increase the mean on dataset \textit{Taxi} because the relationship under different datasets is similar regardless of the attacker's goal is increasing or decreasing the mean.

The experimental results are shown in Figure~\ref{}. Overall, the results show that when the attack bypasses the detection (i.e., the p-value is larger than the default $\alpha$), the mean gain is also low and cannot significantly skew the estimated mean. One reason is that the number of compromised users is small when attack is stealthy. In particular, the attack can bypass the detection when $\beta = 1\%$ in our experiments. Additionally, the p-value is significantly greater than our specified $\alpha$ when there is no attack, and for the attack that can be detected, we observe that its p-values are close to zero. The large gap between two p-values indicates our detection can effectively capture the attack.
